Multivariate Functional Linear Discriminant Analysis: An Application to Inflammatory Bowel Disease Classification

Inflammatory Bowel Disease (IBD), including Crohn's Disease (CD) and Ulcerative Colitis (UC), presents significant public health challenges due to its complex etiology. Motivated by the IBD study of the Integrative Human Microbiome Project, our objective is to identify microbial pathways that distinguish between CD, UC and non-IBD over time. Most current research relies on simplistic analyses that examine one variable or time point at a time, or address binary classification problems, limiting our understanding of the dynamic interactions within the microbiome over time. To address these limitations, we develop a novel functional data analysis approach for discriminant analysis of multivariate functional data that can effectively handle multiple high-dimensional predictors, sparse time points, and categorical outcomes. Our method seeks linear combinations of functions (i.e., discriminant functions) that maximize separation between two or more groups over time. We impose a sparsity-inducing penalty when estimating the discriminant functions, allowing us to identify relevant discriminating variables over time. Applications of our method to the motivating data identified microbial features related to mucin degradation, amino acid metabolism, and peptidoglycan recognition, which are implicated in the progression and development of IBD. Furthermore, our method highlighted the role of multiple vitamin B deficiencies in the context of IBD. By moving beyond traditional analytical frameworks, our innovative approach holds the potential for uncovering clinically meaningful discoveries in IBD research.

==> Var/pathway_explanation.tex <==
\subsection{Microbial Pathways Discriminating Between IBD and non-IBD}
The microbial pathways selected involve specific gut bacteria, such as \textit{Blautia} \citep{liu2021blautia}, \textit{Ruminococcus} \citep{henke2019ruminococcus}, \textit{Alistipes} \citep{parker2020genus}, and \textit{Bacteroides} \citep{zhou2016lower}, highlight the role of microbial composition and dysbiosis in IBD. Amino acid metabolism pathways are intricately linked to key processes affecting IBD status by influencing protein synthesis, immune regulation, and mucosal health, including those for branched-chain amino acids \citep{vidal2017dietary}, histidine \citep{wu2022role}, isoleucine \citep{coeffier2010potential}, glutamate \citep{li2014glutamate}, and glutamine \citep{severo2021effects}. Short-chain fatty acid (SCFA) production pathways, such as butanoate/butyrate fermentation \citep{basson2016mucosal}, are crucial for maintaining epithelial integrity, modulating inflammation, and providing energy to colonocytes. Carbohydrate degradation pathways \citep{cheng2020review} affect the availability of fermentable substrates and SCFA production, influencing the function of the gut barrier and immune responses. The fatty acid metabolism pathways \citep{heimerl2006alterations} alter the composition and fluidity of the cell membrane, affecting the adherence, colonization, and immune interactions of bacteria.

In addition, pathways involved in vitamin and cofactor biosynthesis \citep{ghishan2017vitamins}, such as those of Vitamin B5 \citep{mikkelsen2019vitamin} and menaquinone \citep{dash2021metagenomic}, are essential for microbial metabolism and gut health. Nucleotide biosynthesis \citep{morgan2012dysfunction} and salvage pathways are vital for DNA and RNA synthesis, affecting cell growth and division, which in turn impact microbial stability and immune responses. Stress response pathways, like ppGpp biosynthesis \citep{paramsothy2019specific}, influence bacterial survival and interactions with the host immune system. Lipid and membrane metabolism pathways, such as phosphatidylcholine acyl editing \citep{shores2011new}, affect bacterial cell membrane integrity and host interactions. Lastly, nitrogen metabolism pathways, including citrulline biosynthesis \citep{middleton1993increased}, have an impact on nitric oxide production and gut mucosal health. Together, these pathways contribute to a balanced gut microbiome, proper metabolic functions, and a regulated immune system, all of which are critical in preventing or managing IBD. They influence immune modulation, maintain the integrity of the intestinal barrier, ensure energy production, and regulate inflammatory responses, underscoring their importance in distinguishing IBD patients from healthy individuals.

\subsection{Microbial Pathways Discriminating between CD, UC, and non-IBD}
There are 59 microbiome pathways selected by SFLDA that can distinguish between UC, CD, and non-IBD patients. For instance, \textit{Akkermansia muciniphila} \citep{zheng2023role} is known for degrading mucin, a gut lining component, and its presence can indicate differences in mucin degradation, which is more pronounced in UC. Several metabolic pathways involve \textit{Alistipes putredinis}, a microbial species associated with amino acid metabolism and anti-inflammatory properties \citep{parker2020genus} where these pathways influence the distinct inflammatory and metabolic environments in UC and CD. By modulating amino acid metabolism, \textit{A. putredinis} may play a role in immune regulation and mucosal health, potentially contributing to differences in inflammation between UC and CD. The N10-formyl-tetrahydrofolate biosynthesis pathway \citep{leibovitzh2022altered} is crucial for DNA synthesis and repair, and disruptions can indicate altered microbial metabolism linked to inflammation and tissue repair mechanisms further differing between UC and CD from non-IBD. Glycolysis pathways (III and IV) \citep{bos2020metabolic} are central to energy metabolism, and variations here can reflect differences in microbial community composition and energy requirements. Coenzyme A biosynthesis (II) \citep{ellestad1976pantothenic} is essential for fatty acid metabolism and energy production, and changes in this pathway might indicate differences in lipid metabolism and energy utilization. The dTDP-L-rhamnose biosynthesis \citep{li2022capsular} pathway involves sugar component synthesis for bacterial cell walls, with variations reflecting differences in bacterial populations and structural integrity. Histidine metabolism \citep{wu2022role} is linked to inflammatory histamine production, and differences in these pathways might indicate varying inflammatory responses. Incomplete reductive TCA cycle pathways \citep{ooi2011gc} involve intermediary metabolism, differing based on microbial community composition and the host's metabolic state. Pantothenate \citep{schalich2024human} and coenzyme A biosynthesis \citep{ellestad1976pantothenic} are critical for fatty acid metabolism and energy production, reflecting variations in energy metabolism and microbial composition. Pyruvate fermentation to acetate and lactate indicates microbial fermentation processes, reflecting differences in microbial populations and activity. The superpathway of sulfur oxidation \citep{teigen2019dietary} is important for gut health, and differences here might indicate variations in microbial sulfur metabolism, impacting inflammation and oxidative stress. Peptidoglycan biosynthesis \citep{fernandez2011anti} and maturation are involved in bacterial cell wall synthesis, with variations indicating differences in microbial community structure. Thiamin biosynthesis \citep{costantini2013thiamine} and salvage pathways are crucial for microbial and host metabolism, reflecting variations in vitamin B1 \citep{mikkelsen2019vitamin} availability and utilization. L-isoleucine and L-valine biosynthesis pathways \citep{xie2021systematic} are essential for protein synthesis and microbial growth, indicating distinct microbial communities and metabolic states. The superpathway of menaquinol-8 biosynthesis \citep{dash2021metagenomic} is involved in vitamin K2 production, impacting blood clotting and bone health, with differences indicating variations in microbial vitamin K2 production. Peptidoglycan \citep{fernandez2011anti} and other sugar biosynthesis pathways involve bacterial cell wall component synthesis, reflecting differences in microbial structural integrity and immune interactions. Purine ribonucleosides degradation is involved in nucleotide metabolism, with differences reflecting variations in microbial nucleotide turnover and host-microbiota interactions. Finally, gluconeogenesis and anaerobic energy metabolism pathways \citep{eriksson1983splanchnic, roediger1980colonic} are key for energy production, indicating distinct metabolic adaptations of the gut microbiota. Examining these pathways provides insights into the distinct metabolic and microbial landscapes associated with UC, CD, and non-IBD conditions, leading to better diagnostic and therapeutic strategies.


